MURA: Large Dataset for Abnormality Detection in Musculoskeletal Radiographs

We introduce MURA, a large dataset of musculoskeletal radiographs containing 40,561 images from 14,863 studies, where each study is manually labeled by radiologists as either normal or abnormal. To evaluate models robustly and to get an estimate of radiologist performance, we collect additional labels from six board-certified Stanford radiologists on the test set, consisting of 207 musculoskeletal studies. On this test set, the majority vote of a group of three radiologists serves as gold standard. We train a 169-layer DenseNet baseline model to detect and localize abnormalities. Our model achieves an AUROC of 0.929, with an operating point of 0.815 sensitivity and 0.887 specificity. We compare our model and radiologists on the Cohen's kappa statistic, which expresses the agreement of our model and of each radiologist with the gold standard. Model performance is comparable to the best radiologist performance in detecting abnormalities on finger and wrist studies. However, model performance is lower than best radiologist performance in detecting abnormalities on elbow, forearm, hand, humerus, and shoulder studies. We believe that the task is a good challenge for future research. To encourage advances, we have made our dataset freely available at https://stanfordmlgroup.github.io/competitions/mura .

==> experiments.tex <==
\section{Experiments}
We investigate the impact of a few features of our data collection, preprocessing and training on the performance of the model.

\subsection{Data Augmentation}
We explore the effect of data augmentations on the performance of the model. We hypothesize that with augmentation, the network can generalize better: rotated films are abundant in the dataset, and flipped films can be interpreted as films from other anatomical side of the body. Using identical model architectures, training procedures, and hyperparameter choices, we investigate model performance with and without horizontal flips and rotations (at 10, 20, and 30 degrees).

We find that both flipping and rotating augmentations improve the performance of the model. Without any data augmentation, the average F1 score across all classes is  (). Flipping by itself increases the F1 score to () and rotation by itself increases the F1 score to () With both augmentations, validation F1 increases to ().

\subsection{Training Set Size}
We investigate the importance of the scale of the data to the performance of the model. In particular, we train models on smaller subsets of the training set (1/2 1/4, 1/8, 1/16, 1/32) and report the AUCs on our validation set. We use identical model architectures, training procedures, and hyperparameter choices across the models.

We find that when we reduce our training set size by a factor of 2, validation F1 drops by a factor of (), from () to (). With further reductions in training size, the validation AUC drops by larger factors ().

We recognize that this analysis does have its limitations: a smaller model or a less regularized model would be less sensitive to training set size, while a model that is not pretrained would be more sensitive. However, the analysis does allow us to estimate the effect of dataset scale on performance on the abnormality detection task.

% Table 3: ROC-AUCs by Experiment by Condition
\begin{table}[!htb]
  \caption{F1s by Experiment Condition by Label}
  
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|l|r}
      \hline
      Experiment & Condition & F1 score (test set) \\
      \hline
      Training Size & 1/1x & 0.8267 \\
      \hline
      Training Size & 1/2x & 0.8389\\
      \hline
      Training Size & 1/4x & 0.8041\\
      \hline
      Training Size & 1/8x & 0.7894\\
      \hline
      Training Size & 1/16x & 0.7774\\
      \hline
      Training Size & 1/32x & 0.7237\\
      \hline
    \end{tabular}
  }
\end{table}

\subsection{Loss Function Weighting}
It has been well established that class imbalance can have significant detrimental effect on training of traditional classifiers \cite{Buda2017}. We investigate the effect of removing the class-weighted loss on the performance of our model.

We find that removing the weighting is detrimental to the performance of the model. We also observe that in highly unbalanced classes (wrist), the difference is more pronounced ().
